Inference of genetic networks from time course expression data using functional regression with lasso penalty

Statistical inference of genetic regulatory networks is essential for understanding temporal interactions of regulatory elements inside the cells. For inferences of large networks, identification of network structure is typical achieved under the assumption of sparsity of the networks. When the number of time points in the expression experiment is not too small, we propose to infer the parameters in the ordinary differential equations using the techniques from functional data analysis (FDA) by regarding the observed time course expression data as continuous-time curves. For networks with a large number of genes, we take advantage of the sparsity of the networks by penalizing the linear coefficients with a L_1 norm. The ability of the algorithm to infer network structure is demonstrated using the cell-cycle time course data for Saccharomyces cerevisiae.

==> papers <==
@article{
abramovich04,
   Author = {Abramovich, F. and Amato, U. and Angelini, C.},
   Title = {On optimality of Bayesian wavelet estimators},
   Journal = {Scandinavian Journal of Statistics},
   Volume = {31},
   Number = {2},
   Pages = {217-234},
      Year = {2004} }



@article{
abramovich06,
   Author = {Abramovich, F. and Benjamini, Y. and Donoho, D. L. and Johnstone, I. M.},
   Title = {Adapting to unknown sparsity by controlling the false discovery rate},
   Journal = {Annals of Statistics},
   Volume = {34},
   Number = {2},
   Pages = {584-653},
      Year = {2006} }



@article{
abramovich98,
   Author = {Abramovich, F. and Sapatinas, T. and Silverman, B. W.},
   Title = {Wavelet thresholding via a Bayesian approach},
   Journal = {Journal of the Royal Statistical Society Series B-Statistical Methodology},
   Volume = {60},
   Pages = {725-749},
   Note = {Part 4},
      Year = {1998} }



@article{
andrieu05,
   Author = {Andrieu, C. and Moulines, E. and Priouret, P.},
   Title = {Stability of stochastic approximation under verifiable conditions},
   Journal = {Siam Journal on Control and Optimization},
   Volume = {44},
   Number = {1},
   Pages = {283-312},
      Year = {2005} }



@article{
bansal06,
   Author = {Bansal, M. and Della Gatta, G. and di Bernardo, D.},
   Title = {Inference of gene regulatory networks and compound mode of action from time course gene expression profiles},
   Journal = {Bioinformatics},
   Volume = {22},
   Number = {7},
   Pages = {815-822},
      Year = {2006} }



@article{
barron99,
   Author = {Barron, A. and Schervish, M. J. and Wasserman, L.},
   Title = {The consistency of posterior distributions in nonparametric problems},
   Journal = {Annals of Statistics},
   Volume = {27},
   Number = {2},
   Pages = {536-561},
      Year = {1999} }



@article{
bishop98,
   Author = {Bishop, Christopher M. and Svensen, Markus and Williams, Christopher K. I.},
   Title = {GTM: The Generative Topographic Mapping},
   Journal = {Neural Computation},
   Volume = {10},
   Number = {1},
   Pages = {215-234},
      Year = {1998} }



@article{
blackwell62,
   Author = {Blackwell, D. and Dubins, L.},
   Title = {Merging of opinions with increasing information},
   Journal = {Annals of Mathematical Statistics},
   Volume = {33},
   Pages = {882-886},
      Year = {1962} }



@article{
brown96,
   Author = {Brown, L. D. and Low, M. G.},
   Title = {Asymptotic equivalence of nonparametric regression and white noise},
   Journal = {Annals of Statistics},
   Volume = {24},
   Number = {6},
   Pages = {2384-2398},
      Year = {1996} }



@article{
cappe04,
   Author = {Cappe, O. and Guillin, A. and Marin, J. M. and Robert, C. P.},
   Title = {Population Monte Carlo},
   Journal = {Journal of Computational and Graphical Statistics},
   Volume = {13},
   Number = {4},
   Pages = {907-929},
      Year = {2004} }



@article{
chen05,
   Author = {Chen, K. C. and Wang, T. Y. and Tseng, H. H. and Huang, C. Y. F. and Kao, C. Y.},
   Title = {A stochastic differential equation model for quantifying transcriptional regulatory network in Saccharomyces cerevisiae},
   Journal = {Bioinformatics},
   Volume = {21},
   Number = {12},
   Pages = {2883-2890},
      Year = {2005} }



@article{
delyon99,
   Author = {Delyon, B. and Lavielle, V. and Moulines, E.},
   Title = {Convergence of a stochastic approximation version of the EM algorithm},
   Journal = {Annals of Statistics},
   Volume = {27},
   Number = {1},
   Pages = {94-128},
      Year = {1999} }



@article{
diaconis86,
   Author = {Diaconis, P. and Freedman, D.},
   Title = {On the Consistency of Bayes Estimates},
   Journal = {Annals of Statistics},
   Volume = {14},
   Number = {1},
   Pages = {1-26},
      Year = {1986} }



@article{
donoho94,
   Author = {Donoho, D. L. and Johnstone, I. M.},
   Title = {Ideal Spatial Adaptation by Wavelet Shrinkage},
   Journal = {Biometrika},
   Volume = {81},
   Number = {3},
   Pages = {425-455},
      Year = {1994} }



@article{
donoho95a,
   Author = {Donoho, D. L. and Johnstone, I. M.},
   Title = {Adapting to unknown smoothness via wavelet shrinkage},
   Journal = {Journal of the American Statistical Association},
   Volume = {90},
   Number = {432},
   Pages = {1200-1224},
      Year = {1995} }



@article{
donoho98,
   Author = {Donoho, D. L. and Johnstone, I. M.},
   Title = {Minimax estimation via wavelet shrinkage},
   Journal = {Annals of Statistics},
   Volume = {26},
   Number = {3},
   Pages = {879-921},
      Year = {1998} }



@article{
donoho95b,
   Author = {Donoho, D. L. and Johnstone, I. M. and Kerkyacharian, G. and Picard, D.},
   Title = {Wavelet Shrinkage - Asymptopia},
   Journal = {Journal of the Royal Statistical Society Series B-Methodological},
   Volume = {57},
   Number = {2},
   Pages = {301-337},
      Year = {1995} }



@article{
donoho96,
   Author = {Donoho, D. L. and Johnstone, I. M. and Kerkyacharian, G. and Picard, D.},
   Title = {Density estimation by wavelet thresholding},
   Journal = {Annals of Statistics},
   Volume = {24},
   Number = {2},
   Pages = {508-539},
      Year = {1996} }



@article{
douc07,
   Author = {Douc, R. and Guillin, A. and Marin, J. M. and Robert, C. P.},
   Title = {Convergence of adaptive mixtures of importance sampling schemes},
   Journal = {Annals of Statistics},
   Volume = {35},
   Number = {1},
   Pages = {420-448},
      Year = {2007} }



@article{
efron04,
   Author = {Efron, B. and Hastie, T. and Johnstone, I. and Tibshirani, R.},
   Title = {Least angle regression},
   Journal = {Annals of Statistics},
   Volume = {32},
   Number = {2},
   Pages = {407-451},
      Year = {2004} }



@article{
friedman04,
   Author = {Friedman, N.},
   Title = {Inferring cellular networks using probabilistic graphical models},
   Journal = {Science},
   Volume = {303},
   Number = {5659},
   Pages = {799-805},
      Year = {2004} }



@article{
gardner03,
   Author = {Gardner, T. S. and di Bernardo, D. and Lorenz, D. and Collins, J. J.},
   Title = {Inferring genetic networks and identifying compound mode of action via expression profiling},
   Journal = {Science},
   Volume = {301},
   Number = {5629},
   Pages = {102-105},
      Year = {2003} }



@article{
ghosal00,
   Author = {Ghosal, S. and Ghosh, J. K. and Van der Vaart, A. W.},
   Title = {Convergence rates of posterior distributions},
   Journal = {Annals of Statistics},
   Volume = {28},
   Number = {2},
   Pages = {500-531},
      Year = {2000} }



@article{
ghosal07,
   Author = {Ghosal, S. and Van Der Vaart, A.},
   Title = {Convergence rates of posterior distributions for noniid observations},
   Journal = {Annals of Statistics},
   Volume = {35},
   Number = {1},
   Pages = {192-223},
      Year = {2007} }



@article{
haario01,
   Author = {Haario, H. and Saksman, E. and Tamminen, J.},
   Title = {An adaptive Metropolis algorithm},
   Journal = {Bernoulli},
   Volume = {7},
   Number = {2},
   Pages = {223-242},
      Year = {2001} }



@article{
triebel05,
   Author = {Haroske, D. A. and Triebel, H.},
   Title = {Wavelet bases and entropy numbers in weighted function spaces},
   Journal = {Mathematische Nachrichten},
   Volume = {278},
   Number = {1-2},
   Pages = {108-132},
      Year = {2005} }



@article{
hirose08,
   Author = {Hirose, Osamu and Yoshida, Ryo and Imoto, Seiya and Yamaguchi, Rui and Higuchi, Tomoyuki and Charnock-Jones, D. Stephen and Print, Cristin and Miyano, Satoru},
   Title = {Statistical inference of transcriptional module-based gene networks from time course gene expression profiles by using state space models},
   Journal = {Bioinformatics},
   Pages = {932-942},
   Volume = {24},
   Number = {7},
      Year = {2008} }



@article{
hoff07,
   Author = {Hoff, Peter D.},
   Title = {Model Averaging and Dimension Selection for the Singular Value Decomposition},
   Journal = {Journal of the American Statistical Association},
   Volume = {102},
   Pages = {674-685},
      Year = {2007} }



@article{
hunter04,
   Author = {Hunter, D. R. and Lange, K.},
   Title = {A tutorial on MM algorithms},
   Journal = {American Statistician},
   Volume = {58},
   Number = {1},
   Pages = {30-37},
      Year = {2004} }



@article{
jaakkola94,
   Author = {Jaakkola, T. and Jordan, M. I. and Singh, S. P.},
   Title = {ON THE CONVERGENCE OF STOCHASTIC ITERATIVE DYNAMIC-PROGRAMMING ALGORITHMS},
   Journal = {Neural Computation},
   Volume = {6},
   Number = {6},
   Pages = {1185-1201},
      Year = {1994} }



@article{
johnstone05,
   Author = {Johnstone, I. M. and Silverman, B. W.},
   Title = {Empirical Bayes selection of wavelet thresholds},
   Journal = {Annals of Statistics},
   Volume = {33},
   Number = {4},
   Pages = {1700-1752},
      Year = {2005} }



@article{
kleijn06,
   Author = {Kleijn, B. J. K. and Van der Vaart, A. W.},
   Title = {Misspecification in infinite-dimensional Bayesian statistics},
   Journal = {Annals of Statistics},
   Volume = {34},
   Number = {2},
   Pages = {837-877},
      Year = {2006} }



@article{
lawrence05,
   Author = {Lawrence, Neil},
   Title = {Probabilistic Non-linear Principal Component Analysis with Gaussian Process Latent Variable Models},
   Journal = {J. Mach. Learn. Res.},
   Volume = {6},
   Pages = {1783-1816},
   Keywords = {pca},
   Year = {2005} }



@article{
nam07,
   Author = {Nam, D. and Yoon, S. H. and Kim, J. F.},
   Title = {Ensemble learning of genetic networks from time-series expression data},
   Journal = {Bioinformatics},
   Volume = {23},
   Number = {23},
   Pages = {3225-3231},
      Year = {2007} }




@article{
nickl07,
   Author = {Nickl, R. and Potscher, B. M.},
   Title = {Bracketing metric entropy rates and empirical central limit theorems for function classes of Besov- and Sobolev-type},
   Journal = {Journal of Theoretical Probability},
   Volume = {20},
   Number = {2},
   Pages = {177-199},
      Year = {2007} }



@article{
rosset07,
   Author = {Rosset, S. and Zhu, J.},
   Title = {Piecewise linear regularized solution paths},
   Journal = {Annals of Statistics},
   Volume = {35},
   Number = {3},
   Pages = {1012-1030},
      Year = {2007} }



@article{
schwartz65,
   Author = {Schwartz, L.},
   Title = {On Bayes Procedures},
   Journal = {Z. Wahrsch. Verw. Gabiete},
   Volume = {4},
   Pages = {10-26},
      Year = {1965} }



@article{
shenwong01,
   Author = {Shen, X. T. and Wasserman, L.},
   Title = {Rates of convergence of posterior distributions},
   Journal = {Annals of Statistics},
   Volume = {29},
   Number = {3},
   Pages = {687-714},
      Year = {2001} }



@article{
simon01,
   Author = {Simon, I. and Barnett, J. and Hannett, N. and Harbison, C. T. and Rinaldi, N. J. and Volkert, T. L. and Wyrick, J. J. and Zeitlinger, J. and Gifford, D. K. and Jaakkola, T. S. and Young, R. A.},
   Title = {Serial regulation of transcriptional regulators in the yeast cell cycle},
   Journal = {Cell},
   Volume = {106},
   Number = {6},
   Pages = {697-708},
      Year = {2001} }



@article{
spellman98,
   Author = {Spellman, P. T. and Sherlock, G. and Zhang, M. Q. and Iyer, V. R. and Anders, K. and Eisen, M. B. and Brown, P. O. and Botstein, D. and Futcher, B.},
   Title = {Comprehensive identification of cell cycle-regulated genes of the yeast Saccharomyces cerevisiae by microarray hybridization},
   Journal = {Molecular Biology of the Cell},
   Volume = {9},
   Number = {12},
   Pages = {3273-3297},
      Year = {1998} }



@article{
teixeira06,
   Author = {Teixeira, M. C. and Monteiro, P. and Jain, P. and Tenreiro, S. and Fernandes, A. R. and Mira, N. P. and Alenquer, M. and Freitas, A. T. and Oliveira, A. L. and Sa-Correia, I.},
   Title = {The YEASTRACT database: a tool for the analysis of transcription regulatory associations in Saccharomyces cerevisiae},
   Journal = {Nucleic Acids Research},
   Volume = {34},
   Pages = {D446-D451},
      Year = {2006} }



@article{
tibshiranni96,
   Author = {Tibshirani, R.},
   Title = {Regression shrinkage and selection via the Lasso},
   Journal = {Journal of the Royal Statistical Society Series B-Methodological},
   Volume = {58},
   Number = {1},
   Pages = {267-288},
      Year = {1996} }



@article{
tipping99,
   Author = {Tipping, Michael E. and Bishop, Christopher M.},
   Title = {Mixtures of Probabilistic Principal Component Analyzers},
   Journal = {Neural Computation},
   Volume = {11},
   Number = {2},
   Pages = {443-482},
      Year = {1999} }



@article{
tippingpca99,
   Author = {Tipping, Michael E. and Bishop, Christopher M.},
   Title = {Probabilistic Principal Component Analysis},
   Journal = {Journal of the Royal Statistical Society: Series B (Statistical Methodology)},
   Volume = {61},
   Number = {3},
   Pages = {611-622},
      Year = {1999} }



@article{
tsitsiklis94,
   Author = {Tsitsiklis, J. N.},
   Title = {ASYNCHRONOUS STOCHASTIC-APPROXIMATION AND Q-LEARNING},
   Journal = {Machine Learning},
   Volume = {16},
   Number = {3},
   Pages = {185-202},
      Year = {1994} }



@article{
walker03,
   Author = {Walker, S.},
   Title = {On sufficient conditions for Bayesian consistency},
   Journal = {Biometrika},
   Volume = {90},
   Number = {2},
   Pages = {482-488},
      Year = {2003} }



@article{
walker04,
   Author = {Walker, S.},
   Title = {New approaches to Bayesian consistency},
   Journal = {Annals of Statistics},
   Volume = {32},
   Number = {5},
   Pages = {2028-2043},
      Year = {2004} }



@article{
walker07,
   Author = {Walker, S.  and Lijoi, A.  and Pr\"unster, I.},
   Title = {On rates of convergence for posterior distributions in infinite-dimensional models},
   Journal = {Annals of Statistics},
   Volume = {35},
   Number = {2},
   Pages = {738-746},
      Year = {2007} }



@article{
webb96,
   Author = {Webb, Andrew R.},
   Title = {An approach to non-linear principal components analysis using radially symmetric kernel functions},
   Journal = {Statistics and Computing},
   Volume = {6},
   Number = {2},
   Pages = {159-168},
 Year = {1996} }



@article{
yu04,
   Author = {Yu, J. and Smith, V. A. and Wang, P. P. and Hartemink, A. J. and Jarvis, E. D.},
   Title = {Advances to Bayesian network inference for generating causal networks from observational biological data},
   Journal = {Bioinformatics},
   Volume = {20},
   Number = {18},
   Pages = {3594-3603},
      Year = {2004} }



@article{
zhao00,
   Author = {Zhao, L. H.},
   Title = {Bayesian aspects of some nonparametric problems},
   Journal = {Annals of Statistics},
   Volume = {28},
   Number = {2},
   Pages = {532-552},
      Year = {2000} }



@article{
zou06,
   Author = {Zou, H.},
   Title = {The adaptive lasso and its oracle properties},
   Journal = {Journal of the American Statistical Association},
   Volume = {101},
   Number = {476},
   Pages = {1418-1429},
      Year = {2006} }




